GreediRIS: Scalable Influence Maximization using Distributed Streaming Maximum Cover

Influence maximization--the problem of identifying a subset of k influential seeds (vertices) in a network--is a classical problem in network science with numerous applications. The problem is NP-hard, but there exist efficient polynomial time approximations. However, scaling these algorithms still remain a daunting task due to the complexities associated with steps involving stochastic sampling and large-scale aggregations. In this paper, we present a new parallel distributed approximation algorithm for influence maximization with provable approximation guarantees. Our approach, which we call GreediRIS, leverages the RandGreedi framework--a state-of-the-art approach for distributed submodular optimization--for solving a step that computes a maximum k cover. GreediRIS combines distributed and streaming models of computations, along with pruning techniques, to effectively address the communication bottlenecks of the algorithm. Experimental results on up to 512 nodes (32K cores) of the NERSC Perlmutter supercomputer show that GreediRIS can achieve good strong scaling performance, preserve quality, and significantly outperform the other state-of-the-art distributed implementations. For instance, on 512 nodes, the most performant variant of GreediRIS achieves geometric mean speedups of 28.99x and 36.35x for two different diffusion models, over a state-of-the-art parallel implementation. We also present a communication-optimized version of GreediRIS that further improves the speedups by two orders of magnitude.

==> abstract.tex <==

%The vices of life: get greedy, get lazy, and distribute work 

%% 150 word limit for linklings 


Influence maximization---the problem of identifying a subset of $k$ influential seeds (vertices) in a network---is a classical problem in network science with numerous applications. The problem is NP-hard, but there exist efficient polynomial time approximations. However, scaling these algorithms still remain a daunting  task due to the complexities associated with steps involving stochastic sampling and large-scale aggregations. 
%Consequently, sequential approaches could take hours to execute on modest-sized inputs.
%In this paper, we revisit parallelizing influence maximization through the lens of distributed submodular optimization. 
In this paper, we present a new parallel distributed approximation algorithm for influence maximization with provable approximation guarantees. Our approach, which we call \greedimm, leverages the \randgreedi{} framework---a state-of-the-art approach for distributed submodular optimization---for solving a step that computes a maximum $k$ cover. \greedimm{} combines distributed and streaming models of computations, along with pruning techniques, to effectively address the communication bottlenecks of the algorithm.
Experimental results on up to 512 nodes (32K cores) of the NERSC Perlmutter supercomputer show that \greedimm{} can achieve good strong scaling performance, preserve quality, and significantly outperform the other state-of-the-art distributed implementations.
For instance, on 512 nodes, the most performant variant of \greedimm{} achieves geometric mean speedups of 28.99$\times$ and 36.35$\times$ for two different diffusion models, over a state-of-the-art parallel implementation. We also present a communication-optimized version of \greedimm{} that further improves the speedups by two orders of magnitude.
% \rb{changed the numbers here}
% \mh{GreediRIS-trunc is too long a name. you can shorten it.}


%%%%%%%%%%% short abstract --- <= 150 words

%Influence maximization, a problem of identifying a subset of $k$ influential seeds (vertices) in a network, is a classical problem in network science with numerous scientific applications. While there are efficient approximations for the problem, scaling influence maximization on distributed memory systems remains a daunting task due to the underlying complexities of a stochastic sampling step and large-scale global reductions. In this paper, we present a new scalable distributed algorithm and implementation for influence maximization with provable guarantees. Our approach, which we call GreeDIMM, leverages the GreeDI framework – a state-of-the-art approach for distributed submodular optimization – for solving a step that computes a maximum cover. GreeDIMM uses streaming and nonblocking communications for reducing performance and memory overheads. Experimental results show that GreeDIMM is able to significantly outperform state-of-the-art parallel influence maximization implementations – by reducing time to solution, enhancing problem size reach, and preserving the approximation quality of the solution.



==> figures/plot-receiverbreakdown.tex <==
\begin{figure*}[tbh]
\centering
\begin{subfigure}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{figures/Livejournal_Receiver.pdf}
    \caption{\small LiveJournal: Receiver time breakdown}
    \label{fig:lvjstrong:receiver}
\end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
    \centering
    \includegraphics[width=.8\textwidth]{figures/Wikipedia_Receiver.pdf}
    \caption{\small Wikipedia: Receiver time breakdown}
    \label{fig:wikistrong:receiver}
\end{subfigure}
\vspace{-0.2cm}
%%%%%%%%%%%%%%%%%%%%%
\caption{\small {\em Parallel runtime breakdown} for the receiver process of \greedimm, between its communicating thread and bucketing threads.  
}
    \label{fig:receiverbreakdown}
\end{figure*}

